Managing ML Pipelines: Feature Stores and the Coming Wave of Embedding Ecosystems

The industrial machine learning pipeline requires iterating on model features, training and deploying models, and monitoring deployed models at scale. Feature stores were developed to manage and standardize the engineer's workflow in this end-to-end pipeline, focusing on traditional tabular feature data. In recent years, however, model development has shifted towards using self-supervised pretrained embeddings as model features. Managing these embeddings and the downstream systems that use them introduces new challenges with respect to managing embedding training data, measuring embedding quality, and monitoring downstream models that use embeddings. These challenges are largely unaddressed in standard feature stores. Our goal in this tutorial is to introduce the feature store system and discuss the challenges and current solutions to managing these new embedding-centric pipelines.

==> sections/ml_for_db_2.tex <==
% Outline
% Data Integration:
% - Define
% - Rule based -> ML based (3 min overview of Theo's tutorial basically)
% - Use of static word embeddings
%     - Fuzzy matching search
%     - Dirty data
%     - Transfer learning
% - Pretrained Embedding:
%     - Brunner
%     - Yoliang
% Other Ideas:
%     - Neural DBs
%     - Query
% DB Embeddings

We now discuss how pretrained embeddings have helped address core problems in data management. In particular, as pretrained embeddings allow for accessing semantic knowledge about words and entities, we see that data management subfields such as neural databases~\cite{thorne2020neural}, natural language query processing~\cite{li2020querying}, and cardinality estimation~\cite{marcus2019neo} have seen growth with respect to the incorporation of embeddings. In this tutorial, we decide to focus on one subfield: data integration---the task of integrating varied source data sets into a target format~\cite{cabrera2018dibs}. We highlight data integration systems leveraging pretrained embeddings as well as systems that use the self-supervised methods to produce ``relation embeddings'' for data integration.

% We have seen less growth with the incorporation of pretrained entity embeddings, such as TransE, that are trained over entities in Wikidata. As relational data often contains {\em personalized} or business specific entities that are not represented in common corpuses, there is less utility in using them. To address this, some recent methods are using the same ideas from self-supervised word and entity embedding pretraining to create database specific entity embeddings.

\subsection{Data Integration}
Data integration is the task of extracting structure data, i.e., entities and relations, from heterogeneous collections of unstructured, semi-structured, or structured data~\cite{niu2012deepdive}. Prior approaches were rule based~\cite{brunner2020entity} with some machine learned components using methods such as decision trees or logistic regression~\cite{dong2018data}. Only in the past 5-8 years have pretrained embeddings been incorporated into the pipeline.

% Some of the earliest adoptions were through the use of pretrained word embeddings like word2vec~\cite{mikolov2013efficient}, GloVe~\cite{pennington2014glove}, and fastText~\cite{joulin2016bag} to aid in data discovery. The work of \cite{nargesian2018table} uses fastText embeddings to measure the similarity between two attributes of different tables for finding unionable tables in open data. The work of \cite{fernandez2018seeping} uses GloVe embeddings to automatically link datasets for faster data exploration. Both of these works use the embeddings to calculate an approximate similarity between attributes.

The task of entity matching, finding data instances that refer to the same real-world entity, has seen the widest adoption of the incorporation of pretrained knowledge through embeddings~\cite{mudgal2018deep}. The work of \cite{ebraheem2018distributed} learns a tuple representation for resolution by combining the pretrained words embeddings of each token in a tuple with a LSTM. They handle out-of-vocabulary words through {\em retrofitting} where new words are assigned embeddings by averaging known embeddings of words that co-occur in a tuple. They find the use of word embeddings improves performance over hand-crafted models by up to 8 F1 points with less engineer effort. The works of \cite{thirumuruganathan2018reuse, kasai2019low} also leverage word embeddings, taking a similar approach as \cite{ebraheem2018distributed} and generating a tuple embedding from its constituent word embeddings. \cite{thirumuruganathan2018reuse} and \cite{kasai2019low} both highlight the challenge of out-of-domain words, with \cite{kasai2019low} using fastText character embeddings to alleviate this problem, and the reduced effort in using pretrained embeddings as they allow for knowledge transfer from larger corpuses. \cite{mudgal2018deep} notes that the benefit of pretrained embeddings diminishes on highly specialized domains. 

% zhao2019auto learns attribute-level entity matching models taht can easily be turned into table level entity matching tasks with little egineer effort. They train from scratch character embeddings with a hierarchical model on top to allow for better similarity scores between two attributes.

Lastly, the recent works of \cite{brunner2020entity} and \cite{yuliang2020deep} take advantage of the contextualized language models such as BERT~\cite{devlin2018bert}, RoBERTa~\cite{liu2019roberta}, and XLNet~\cite{yang2019xlnet}. \cite{brunner2020entity} feeds tuples pairs directly into one of these language models and fine tunes it to predict if the tuples are similar or not. They find that not only do language models outperform preexisting deep learning methods from \cite{ebraheem2018distributed} by up to 35 F1 points, especially over dirty data, but is also faster to tune than training a model from scratch as in \cite{ebraheem2018distributed}. \cite{yuliang2020deep} presents the DITTO system. DITTO's architecture is similar to \cite{brunner2020entity} but they present optimizations in the form of adding attribute type tokens, normalizing the textual inputs, and generating augmented training data. DITTO demonstrates similar performance boosts as \cite{brunner2020entity}.

% \subsection{Neural Databases}
% Outside of data integration, there has been a few notable works leveraging pretrained word embeddings. In particular, the NeuralDB project of \cite{thorne2020neural} explores answering queries using the T5~\cite{raffel2019exploring} deep language model. Given the input query and a set of possible answer facts, they train T5 to output the correct answer (similar to standard QA systems). The authors note the scalability challenge with this approach, as the model needs to be given a set of possible output facts, but emphasize the benefit of knowledge transfer to unseen relations by using a pretrained language model.

% The work of \cite{li2020querying} disucsses how to answer "subjective" queries and uses word embeddings for incorporating knowledge of contextual ques in subjective queries.

\subsection{Relation Embeddings}
A recent trend has been to try to build a general purpose pretrained {\em relation} embedding that can, like word embeddings, be used in a variety of downstream integration tasks. The work in \cite{gunther2019retro} learns both a token embedding by retrofitting, taking account of the relationships between attributes, and a node embedding via the DeepWalk method. These are concatenated to generate a tuple representation. \cite{gunther2019retro} shows that their representations can provide lift in standard ML tasks of regression and link prediction. \cite{cappuzzo2020creating} builds a relation embeddings for data integration. Instead of treating a tuple as a sentence and using standard language embedding methods like \cite{zhao2019auto}, they encode the structure of a tuple through a tripartite graph and generate sentences via a random walk. They then use word embedding pretraining methods to learn embeddings for records, attributes, and values. The demonstrate the applicability of these embeddings in downstream tasks of schema matching, entity resolution, and token matching. Both methods highlight the need to incorporate both the attribute values and the structural relationships to learn relation embeddings.
